Astro2020 Science White Paper: A Shocking Shift in Paradigm for Classical Novae

The discovery of GeV gamma-rays from classical novae has led to a reassessment of these garden-variety explosions, and highlighted their importance for understanding radiative shocks, particle acceleration, and dust formation in more exotic, distant transients. Recent collaboration between observers and theorists has revealed that shocks in novae are energetically important, and can even dominate their bolometric luminosity. Shocks may also explain long-standing mysteries in novae such as dust production, super-Eddington luminosities, and `flares' in optical light curves. Here, we highlight the multi-wavelength facilities of the next decade that will further test our nova shock model and fulfill the promise of novae as powerful astrophysical laboratories.

==> Makefile <==
TEXFILE_BASENAME = ChomiukLaura

all: clean $(TEXFILE_BASENAME).pdf

clean: 
	rm -f $(TEXFILE_BASENAME).bbl  $(TEXFILE_BASENAME).pdf $(TEXFILE_BASENAME).ps $(TEXFILE_BASENAME).dvi $(TEXFILE_BASENAME).log $(TEXFILE_BASENAME).aux $(TEXFILE_BASENAME).blg DEADJOE *~ *.bak main_paper.pdf online_material.pdf $(TEXFILE_BASENAME).out $(TEXFILE_BASENAME).teximulated mn2e.bst_backup missfont.log *~

$(TEXFILE_BASENAME).pdf: $(TEXFILE_BASENAME).tex
	# BibTeX and eps figures
	latex $(TEXFILE_BASENAME).tex && latex $(TEXFILE_BASENAME).tex && bibtex $(TEXFILE_BASENAME) && latex $(TEXFILE_BASENAME).tex && latex $(TEXFILE_BASENAME).tex && dvips -o $(TEXFILE_BASENAME).ps $(TEXFILE_BASENAME).dvi && ps2pdf $(TEXFILE_BASENAME).ps && okular $(TEXFILE_BASENAME).pdf
	# No BibTeX
	# This works with .eps figures or when \usepackage[demo]{graphicx} is activated
	#latex $(TEXFILE_BASENAME).tex && latex $(TEXFILE_BASENAME).tex && dvips -o $(TEXFILE_BASENAME).ps $(TEXFILE_BASENAME).dvi && ps2pdf $(TEXFILE_BASENAME).ps && okular $(TEXFILE_BASENAME).pdf
	# This works with .png figures
	#pdflatex $(TEXFILE_BASENAME).tex && pdflatex $(TEXFILE_BASENAME).tex && bibtex $(TEXFILE_BASENAME) && pdflatex $(TEXFILE_BASENAME).tex && pdflatex $(TEXFILE_BASENAME).tex && okular $(TEXFILE_BASENAME).pdf
	
